Cosmology with Love: Measuring the Hubble constant using neutron star universal relations

Gravitational-wave cosmology began in 2017 with the observation of the gravitational waves emitted in the merger of two neutron stars, and the coincident observation of the electromagnetic emission that followed. Although only a $30\%$ measurement of the Hubble constant was achieved, future observations may yield more precise measurements either through other coincident events or through cross correlation of gravitational-wave events with galaxy catalogs. Here, we implement a new way to measure the Hubble constant without an electromagnetic counterpart and through the use of the binary Love relations. These relations govern the tidal deformabilities of neutron stars in an equation-of-state insensitive way. Importantly, the Love relations depend on the component masses of the binary in the source frame. Since the gravitational-wave phase and amplitude depend on the chirp mass in the observer (and hence redshifted) frame, one can in principle combine the binary Love relations with the gravitational-wave data to directly measure the redshift, and thereby infer the value of the Hubble constant. We implement this approach in both real and synthetic data through a Bayesian parameter estimation study in a range of observing scenarios. We find that for the LIGO/Virgo/KAGRA design sensitivity era, this method results in a similar measurement accuracy of the Hubble constant to those of current-day, dark-siren measurements. For third generation detectors, this accuracy improves to $\lesssim 10\%$ when combining measurements from binary neutron star events in the LIGO Voyager era, and to $\lesssim 2\%$ in the Cosmic Explorer era.

==> response.tex <==

\begin{enumerate}
    \item In Eq.~(1), is there any criteria for the choice of the fiducial value of $m_0$?

          \textbf{A}: For practical use, the choice of $m_0$ will be decided by the binary
          masses. While the binary Love $\lambdazero-\lambdak$ relation holds true irrespective of the
          choice of $m_0$, there is a neighborhood around $m_0$ where the expansion of 
          $\lambdatilde(m)$ will be a reasonable approximation. Here, we expand up to
          a finite order i.e., $(1 - m/m_0)^3$, and therefore are limited in the neighborhood
          where the approximation makes sense. 
          We find that with $m_0=1.4\;\msun$, in the interval of
          $(1.2, 1.5)\;\msun$, the upper limit of the error is under 10\%.
          We would also like to point out that for our first step of constraining $\lambdazero$,
          we have to use events for which the redshift, or the source-masses
          are measured independently. Here, since we use GW170817, the choice of $m_0 = 1.4~\msun$
          is such that we are in the mass range for GW170817. In a hypothetical case of GW170817
          having significantly different masses, we would have to choose $m_0$ accordingly.

    \item Just below Eq~(1), ``The $\bar{\lambda}_0^{(0)}-\bar{\lambda}_0^{(k)}$ state that...''
          might be better written as ``The $\bar{\lambda}_0^{(0)}-\bar{\lambda}_0^{(k)}$
          relation states that...''. Similar missings with word ``relation'' also
          apply to the rest of the paper.
          
          \textbf{A}: We thank the referee for pointing this out. We have addressed this in the
          revised draft.
    \item In Eq.~(3), is there any particular reason for a bar symbol over $n$
          in the subscript of $G$?
          
          \textbf{A}: The bar represents an average value corresponding to the mean polytropic number of
          the EoS considered in YY17. In our study, we set it equal to $\bar{n} = 0.743$.  This value was
          taken from Table 2 of YY17. This value was obtained in YY17 by fitting the $\bar{\lambda}_{s}-\bar{\lambda}_{a}$
          relation for various EoS in the Newtonian regime with polytropic relations and then taking the mean
          value of the polytropic index from the fit. 

    \item In the paragraph below Eq.~(3) where the Fig.~1 was first mentioned,
          ``The left and right panels of Fig. 1 show the mass-radius curves...''
          should be corrected as ``The upper and middle panels of Fig. 1 show the
          mass-radius curves...''.
          
          \textbf{A}: This was an oversight. We thank the referee for pointing this out.
          This has been addressed in the revised draft.
          
    \item In the paragraph at the bottom of page 4, what is marginalized
          when setting the prior distribution of each component mass as the
          marginalized posterior distribution obtained for the component masses
          from LV19?
          
          \textbf{A}: We mean the single-parameter posterior density, that is
          marginalized over all the other parameters.

    \item In the paragraph at the left-bottom of page 7, the $N_{det}$ is
          chosen as 10, 100, and 1000. Does this paper take into account the
          redshift distribution of the GW events for each $N_{det}$?
          
          \textbf{A}: We do a simplification in this work. The accurate treatment of this step
          requires the knowledge of the rate evolution of BNSs as a function of redshift. 
          While the redshift dependence of binary black hole merger rate has been estimated
          from GW data (in GWTC-2) using several models (\url{https://arxiv.org/pdf/2010.14533.pdf}),
          the lack of confirmed BNS mergers and their relatively closer discovery distances imply
          that the rate evolution of BNSs is not strongly constrained yet. Here, in Fig. 3,
          we distribute the binaries considering a $\sim \dl^2$ prior (uniform in volume).
          However, we have added a new Appendix D in the revised manuscript:
          \textit{Considering alternative redshift priors}, where we have
          verified that alternative, physically motivated choices don't affect our result
          for {\hubble}. In the appendix, we consider two cases for the Cosmic Explorer era as
          an example -- 1) the rate is uniform in comoving volume, and 2) the rate follows cosmic star 
          formation history. Practically, this means that we re-weight the luminosity distances of the
          recovered simulations, from our ensemble in Sec.~\ref{sec:hubble}, based on the
          redshift priors of the two models i.e., the contour map in Fig. 3 changes. This is shown
          in the bottom panel of Fig.~11. Our representative parameter estimation runs shown
          by the grid points, and the counting step is the same as in the
          original draft. We see that the stacked {\hubble} posterior in the top panel of Fig.~11
          is unaffected to the choice of prior used.
          This latter step, described in Sec.~\ref{sec:hubble} is done to avoid having to do several 
          (hundreds) Bayesian parameter estimation runs. 
          
          Due to the lack of constraints on the rate evolution model,
          we believe that our current simplification is justified. However, the prescription in this
          work can easily be re-done as the redshift evolution is better constrained.
          For the other detector eras, the relatively close distances imply that the
          differences in prior choice don't have a significant effect.

    \item How many numbers of the grid points are actually simulated in the
          representative runs for each $N_{det}$ ? Shouldn't we obtain the
          contour map of the right panels of Fig. 3 by first simulating all
          $N_{det}$ events ? How do you obtain the relative probability of the
          contour map before using some fiducial source at certain representative
          points on a grid ?
          
          \textbf{A}: In principle, the representative events considered should be a draw
          from the distribution represented by the heatmap. We should consider
          detected events based on the evolution of the volumetric rate and
          perform Bayesian parameter estimation on all of them. However, the second step would
          be computationally expensive. Thus, practically, we break up the problem in two
          steps --  we estimate the recovered distances and inclinations by simulating the
          GW strain from an ensemble of fiducial systems. We simulate $\sim 10^5$ binary
          systems with fixed masses (same as that we use for parameter estimation), and
          distribute them uniform in sky position, inclination,
          and volume (we also consider other disitrbutions in the new appendix). For each,
          we check whether the strain would be detectable in detectors. Thus, a fraction of the
          total number is detected. The heatmap is a 2D histogram in distance-inclination
          i.e., normalized number count in each bin. We then consider $\mathcal{O}(10)$
          representative systems, shown by the solid grid points, for parameter estimation that
          reasonably cover this distance - inclination plane. We think of the {\hubble}
          measurement from each grid point as representing that from BNSs detected ``around''
          that point. We perform Bayesian parameter estimation on these representative systems.
          We count them based on  what their relative chances of detection should
          be, i.e., the value of the heatmap. Finally, we normalize the count to a ballpark
          number $\Ndet$ that is expected in the detector era (1000 in case of Cosmic Explorer era).

    \item In the paragraph just below Eq.(13), why the SNR of the signal is
          chosen to be larger than 30 (instead of 8 chosen in Fig. 3) in Fisher
          analysis?
          
          \textbf{A}: In this section we are considering Fisher analysis of single
          events. Our aim here is to show that the trends observed in Bayesian parameter
          estimation matches the trends of the Fisher analysis, and to draw comparison
          with the results of Messenger and Read (2012). The choice of the
          SNR threshold was to ensure that the systems we are considering are
          in the Fisher regime i.e. have a ``high'' signal-to-noise. The value 30 was a
          choice made as a proxy for ``high'' SNR, this was also the choice made in YY17. In the revised
          draft, we have extended the x-axis of the top panel of Fig.~4 to match
          the bottom panel. The figure however is to be interpreted with the caveat
          that at larger distances, the Fisher approximation is not necessarily reliable.
          We also mention this in the text and figure caption.

    \item In Fig.~4, the upper panel shows that the relative errors in
          redshift decrease in distance. Is this becaused of larger $N_{det}$ at
          larger distance?
          
          \textbf{A}: This section considers individual events. The analysis is
          similar to Messenger and Read (2012), where it was shown that the
          fractional redshift error for individual events stays almost constant 
          (until a certain redshift) for
          model EoSs (Fig.~1 in \url{https://arxiv.org/pdf/1107.5725.pdf}). Here,
          we show that when we employ the $\lambdazero - \lambdak$ relation and
          consider a Gaussian prior on $\lambdazero$ representing a measurement error,
          the effect is that the fractional error in redshift tends to a constant
          with increasing distance. This shows that the measurement error of
          $\lambdazero$ can affect the measurement of {\hubble} for events
          detected at lower distances, which is something that will be less
          likely given the astrophysical distribution of distances preferring
          more events at larger distances.

    \item The relative errors in $z$ of upper panel of Fig. 4 is at least 30\%,
          and the lower panel shows relative errors in {\hubble} could reach 50.
          How do you draw the conclusion that a prior statistical uncertainty in
          the measurement of $\bar{\Lambda}_0^{(0)}$ will not significantly
          affect the final {\hubble} measurement? Did I mis-interprete the Fig.~4?

          \textbf{A}: In this figure and in Sec.~V, the aim is to compare the relative errors
          obtained using Fisher analysis versus Bayesian parameter estimation on
          individual systems. A major difference in the Fisher vs Bayesian analysis
          is the difference in signal model as mentioned in Sec.~\ref{sec:uncertainties}.
          The Fisher analysis uses a simpler, analytic signal model as mentioned in Sec.~\ref{sec:uncertainties}. 
          Therefore, a difference in the value of the fractional errors
          in redshifts  (y-axis) of the top and bottom panels is expected. In the bottom
          panel, we show the fractional uncertainty for the distance, redshift
          and {\hubble}. We find that the
          distance uncertainty dominates the error for {\hubble} for individual
          events. Regarding the {\hubble} uncertainties, relative errors $\sim 50\%$
          is expected as can be seen from the individual measurements (the dotted curves in Fig. 3).
          The individual likelihoods can be peaked away from the true value and
          can have 90\% confidence region that is not constraining. However,
          combining the measurement brings the error down as shown in the stacked
          likelihood.

    \item In the last paragraph of section V.B, it is mentioned that the
          systematic error will not decrease with more events stacked, which is
          roughly 10\% in H0 measurements as seen from the band region of Fig.~5.
          Is this also true for a redshift-distributed $N_{det}(z)$ (namely
          larger $N_{det}$ for larger distance)?
          
          \textbf{A}: In Sec.~V, we only consider single events. We take the
          expression of $\lambdatilde(m)$ parameterized by the $\lambdazero - \lambdak$
          relation, and introduce an ad-hoc bias in the value of $\lambdazero$.
          The resulting bias in $H_0$ is plotted in the shading -- it will be different
          depending on the masses of system, the shading is an envelope when
          we vary the masses. Supposing there was a bias in $\lambdazero$, similar to the value
          considered here, the inferred $H_0$ from individual events will suffer from a bias
          depending on their distance. However, since this bias is expected to be there for
          all observed systems, the effect will not average out with increasing statistics.
\end{enumerate}
